Diamond pixel detector for beam profile monitoring in COMET experiment at J-PARC

We present the design and initial prototype results of a pixellized proton beam profile monitor for the COMET experiment at J-PARC. The goal of COMET is to look for charged lepton flavor violation by direct muon to electron conversion at a sensitivity of $0^{-19}$. An 8 GeV proton beam pulsed at 100 ns with $10^{10}$ protons/s will be used to create muons through pion production and decay. In the final experiment, the proton flux will be raised to $10^{14}$ protons/sec to increase the sensitivity. These requirements of harsh radiation tolerance and fast readout make diamond a good choice for constructing a beam profile monitor in COMET. We present first results of the characterization of single crystal diamond (scCVD) sourced from a new company, 2a systems Singapore. Our measurements indicate excellent charge collection efficiency and high carrier mobility down to cryogenic temperatures.

==> Makefile <==
# Makefile to create PDF documents from LaTeX-Files 
# Needed software packages: pdflatex, rubber 
# License: No copyright, just do what the heck you want with it 

all: pdf clean 

pdf:
	for file in $$(ls *tex | cut -d \. -f 1) ; do make $$file.pdf ; done 

%.pdf: %.tex
	rubber -m pdftex $< 

clean:
	rm -f *.toc *.aux *.log *.out 

cleanall:
	rm -f *.toc *.pdf *.aux *.log *.out 

.PHONY: all pdf clean cleanall 

.SILENT: pdf

